Comprehensible Counterfactual Explanation on Kolmogorov-Smirnov Test

The Kolmogorov-Smirnov (KS) test is popularly used in many applications, such as anomaly detection, astronomy, database security and AI systems. One challenge remained untouched is how we can obtain an explanation on why a test set fails the KS test. In this paper, we tackle the problem of producing counterfactual explanations for test data failing the KS test. Concept-wise, we propose the notion of most comprehensible counterfactual explanations, which accommodates both the KS test data and the user domain knowledge in producing explanations. Computation-wise, we develop an efficient algorithm MOCHE (for MOst CompreHensible Explanation) that avoids enumerating and checking an exponential number of subsets of the test set failing the KS test. MOCHE not only guarantees to produce the most comprehensible counterfactual explanations, but also is orders of magnitudes faster than the baselines. Experiment-wise, we present a systematic empirical study on a series of benchmark real datasets to verify the effectiveness, efficiency and scalability of most comprehensible counterfactual explanations and MOCHE.

==> Revision_Summary.tex <==
% !TEX root =  main.tex

\setcounter{page}{1}

We are grateful to the reviewers and the meta-reviewer for their constructive and insightful comments. In this revision, we updated more than $40\%$ of the content, including new examples, new baselines, new experiments, adjusted claims, and more clarification and explanation.  We believe that all review comments are addressed in this revision, as summarized here.


% Counterfactual explanation is a formal concept used in the literature of explainable artificial intelligence.
To be consistent with existing studies~\cite{wachter2017counterfactual, meliou2010complexity, fariha2020causality, brundage2020toward, fong2017interpretable, mothilal2020explaining}, in our revision, we use the term \textit{counterfactual explanation}, instead of counterfactual interpretation.

\subsection*{Comments by Meta-reviewer (MR)}

\textbf{MR-Q1:} \textit{``Strengthen experimental study. Generally, the experimental study is not perceived as convincing. Most notably, baselines are missing and quality improvements are often marginal. Moreover, the proposed approach is evaluated on the anomaly detection problem, but uses input information from another anomaly detection algorithm. This is confusing and at the end it's not clear (and quantified) what the added benefit of the proposed approach is with respect to other baselines. Finally, the effect of the preference list quality should be evaluated in more detail.''}

\smallskip\noindent\textbf{Answer:} 
Following your suggestions, we renovate the experiments dramatically. We include new baselines and new experiments. Specifically, we implement three new baseline methods by properly extending the three related studies suggested by Review 1. To avoid any misunderstanding or confusion that our method is an anomaly detection method, in this revision, we redesign our evaluation metrics so that they can better evaluate the performance of all methods. Please refer to our answer to question R1-Q2 for more details.
We also illustrate the effects of preference lists on explanations using a real COVID-19 data set in Example~\ref{ex:lexicographic_order}. In the example, we present and compare the most comprehensible explanations on the same failed KS test that are produced by MOCHE based on two different preference lists, one on regions and the other on age groups.

\medskip

\textbf{MR-Q2:} \textit{``Strengthen motivation and argue clearly for the proposed setting. Most notably, add a convincing motivating example and argue for the use of another anomaly detection method to create the preference list. Also explain better or tone down why you see causal relationships in the counterfactual interpretation of a failed KS test.''}

\smallskip\noindent\textbf{Answer:} First, we extensively revise the introduction to better demonstrate our motivation. A concrete motivation example using a real COVID-19 data set is added to the section. We also clarify our problem setting.

Second, the preference list construction method is not limited to outlier detection methods. 
In Section~\ref{subsec:exp_effective} and Example~\ref{ex:lexicographic_order}, we study two preference lists using regions and age groups, respectively, on the COVID-19 dataset. The two preference lists are irrelevant to outlier detection at all.

%\todel{In our case study on the COVID-19 data set, we study a preference list using population that is irrelevant to outlier detection methods.}

Third, we revise our statements about counterfactual explanation and causality discovery. The counterfactual explanation methods discover relevant and dependent relationships between a set of factors $X$ and a decision $Y$, rather than causal relationships~\cite{wachter2017counterfactual}. Please refer to our answer to question R1-Q6 for more details. 

\medskip

\subsection*{Comments by Reviewer \#1 (R1)}

\textbf{R1-Q1:} \textit{``(W1) The construction of the preference list should be independent from the problem that the KS test is solving''}

\smallskip\noindent\textbf{Answer:} To address this comment, in Example~\ref{ex:lexicographic_order} , we use the KS test to detect differences of distributions of COVID-19 cases in August and September 2020. Using the preference list formed by populations of regions we can obtain explanations about how cases from HAs of large population contribute to the differences. The case study results are presented in Section~\ref{subsec:exp_effective}.  
We also demonstrate that, for users interested in understanding how the distributions of the infected cases are related to age groups, they can use a preference list by sorting all cases in age group descending order.

When a KS test is failed, investigating the outliers in the test set is a common preference of many users~\cite{rabanser2019failing, pinto2019automatic}. 
To capture this preference, for the six datasets in the NAB repository, we apply a time series outlier detection method to generate the preference lists. The outlier detection method and thus the preference lists are independent from the KS test as well. 



\medskip

\textbf{R1-Q2:} \textit{``(W2) For the use case employed in the experimental evaluation, there exist baselines that could be used to compare to''}

\smallskip\noindent\textbf{Answer:}
The previous version mainly uses outlier detection as the example scenario.  We realize that the example there maybe misleading, since the KS test and our counterfactual explanations have much broader applications. To avoid the confusion, in this revision, 
we redesign our evaluation metrics so that they can better evaluate the performance of all methods. 
Moreover, we implement three new baseline methods by extending the studies suggested by Reviewer 1, STOMP~\cite{yeh2016matrix}, Series2Graph~\cite{boniol2020series2graph}, and D3~\cite{10.5555/1182635.1164145}. STOMP and  Series2Graph are time series outlier detection methods. The baseline methods, Extended-STOMP, Extended-Series2Graph, and Extended-D3, generate counterfactual explanations $\mathcal{I}$ by greedily selecting the top $l$ outlying data points (or subsequences) so that $R$ and $T \setminus \mathcal{I}$ can pass the KS test. Unfortunately, the three baseline methods still cannot produce comprehensible counterfactual explanations that satisfy users' preferences. Besides, Extended-STOMP and Extended-Series2Graph can only work on time series. They cannot interpret the failed KS test conducted on the more general data sets, such as the COVID-19 dataset.
In Section~\ref{sec:exp}, we comprehensively compare the performance of our method and the baseline methods. The results show that our method constantly outperforms all baselines in all experiments. 

\medskip

\textbf{R1-Q3:} \textit{``(D1) The way the proposed approach and solution are motivated and built, are not very convincing. The authors describe the use of KS for anomaly detection, and use another anomaly detection algorithm to build the preference list L. So it seems that in order to detect and explain anomalies, their method needs another anomaly detection algorithm. I still believe that proposed approach is interesting. Maybe changing the narrative (motivating example, problem scenario, preference list construction) will address this issue.''}

\smallskip\noindent\textbf{Answer:} 
The reviewer's insight is correct.  Our method aims to interpret why a KS test is failed, rather than anomaly detection. 
We revise the introduction and redesign the experiments to better demonstrate our motivation and evaluate the performance of our methods.
For example, in Section~\ref{sec:exp_effective}, we present a case study about interpreting a failed KS test conducted on the COVID-19 dataset. In that experiment, we use the population descending order of the reported HAs to generate the preference list $L$ of data points (COVID-19 cases) in the test set. This preference list captures a user's interest in understanding how cases from regions of large population contribute to the change of distribution of infected cases.
%\todel{the distribution of COVID-19 cases with respect to HSDAs with different population.}
As shown in our case study in Section~\ref{subsec:exp_effective}, our explanation on the failed KS test 
only includes some COVID-19 cases from the HA with the largest population. In September 2020, the number of infected middle-aged and senior people in the region increased dramatically.
Besides, as discussed in 
Example~\ref{ex:lexicographic_order}, to
%\todel{the distribution of infected cases with respect to age,}
understand how cases in senior age groups contribute to the change of distribution of infected cases,
we can sort all cases in age group descending order and obtain another preference list. In this list, senior people are paid more attention.

\medskip

\textbf{R1-Q4:} \textit{``(D2) The authors now evaluate their method in an anomaly detection setting in time series data, with the proposed approach being used to essentially identify the parts of the time series that constitute the anomalies. They also claim that there are no baselines to compare to. While this is true in what regards the explanation of the KS test, it is not true for identifying time series subsequences that constitute anomalies. Under the current narrative, the authors could apply a time series anomaly detection technique, rank the anomalies by anomaly score, and propose these results as the explanations.''}

\smallskip\noindent\textbf{Answer:} 
To address this comment, we redesign the experiments largely.
Please refer to our answer to the second question (R1-Q2).

\medskip

\textbf{R1-Q5:} \textit{``(D3) Some key references are missing. The last three of the recommended works (or some of them, or one of the methods in the survey below, or even [48,58] of the paper) could be used as a baseline. If the authors want to show that their approach helps in the anomaly detection problem, then they should demonstrate that the use/incorporation of their approach can produce more/better/easier to understand results that other state-of-the-art anomaly detection methods.''}

\smallskip\noindent\textbf{Answer:} 
We add new baselines according to this suggestion. 
Please refer to our answer to the second question (R1-Q2).

\medskip

\textbf{R1-Q6:} \textit{``(D4) Section 3.2 says that "counterfactual interpretation methods describe the causal relationship". Is this truly causality? Please give a reference.''}

\smallskip\noindent\textbf{Answer:} 
The reviewer asks an insightful question.  We revise the statement. The counterfactual explanation methods discover relevant and dependent relationships between a set of factors $X$ and a decision $Y$, rather than causal relationships~\cite{wachter2017counterfactual}.

Counterfactual explanation is an explanation technique proposed by the community of explainable artificial intelligence to interpret algorithmic decisions~\cite{mothilal2020explaining}. The counterfactual explanation methods interpret a decision $Y$ by finding a smallest set of relevant factors $X$, such that changing $X$ can alter the decision $Y$~\cite{moraffah2020causal}. Different from causality analysis~\cite{pearl2018theoretical}, counterfactual explanation cannot identify causalities. It  discovers the relevancy and dependency between the factors $X$ and the decision $Y$~\cite{wachter2017counterfactual}. Counterfactual explanation is widely adopted as an efficient and effective tool to help people understand and handle the algorithmic decisions made in many real world applications~\cite{wachter2017counterfactual, meliou2010complexity, fariha2020causality, brundage2020toward, fong2017interpretable, mothilal2020explaining}. 

A counterfactual explanation on a failed KS test reveals the data points in $T$ that are likely relevant to the failure of the KS test. The identified data points may not be the underlying abnormalities.

%We've revised the corresponding contents in our paper to clarify the concepts.

\medskip

\textbf{R1-Q7:} \textit{``(D5) Section 3.4 says that "each data point has a unique rank in L". I don't agree: it may be the case that an outlier method assigns the same outlying score to two different points.''}

\smallskip\noindent\textbf{Answer:} Our formulation of the most comprehensible counterfactual explanation assumes a preference list of data points in the test set. In general, if two or multiple points have the equivalent preferences, they can be sorted arbitrarily in the preference list.


\medskip

\textbf{R1-Q8:} \textit{``(D6) How different are the preference lists produced by Spectral Residual and Bitmap. You should report this.
''}

\smallskip\noindent\textbf{Answer:} In our experiments, we find that the preference lists constructed by Bitmap and Spectral Residual are very similar to each other, and thus lead to similar explanations on the failed KS tests. Limited by space, we do not report the detailed results with the preference lists constructed by Bitmap. 

\nop{
In addition to outliers, we study two new types of user interest in this revision. 
%\todel{in our updated experiments.}
In Section~\ref{subsec:exp_effective}, we use the population descending order of the reported HAs to generate the preference list $L$ of data points in the test set. 
Example~\ref{ex:lexicographic_order} considers using the age descending order of the infected cases to generate the preference list $L$ of data points in the test set. 
}
%In other words, data points from HSDAs with large population are ranked higher. This preference list captures users' interest in the distribution of COVID-19 cases with respect to HSDAs with different population.

\medskip

\textbf{R1-Q9:} \textit{``(D7) All figures should be enlarged. They are now too small to read.
''}

\smallskip\noindent\textbf{Answer:} All figures are enlarged.

\subsection*{Comments by Reviewer \#2 (R2)}

\textbf{R2-Q1:} \textit{``I *think* that the paper is not in the scope of "very large databases." The indicators for my suspicion: (1) The novelty of the paper is in defining a problem related to a statistical test. (2) The technical part of the paper consists in large parts in exploiting statistical properties. (3) The data sets used have at most a bit more than 100k data points.''}

\smallskip\noindent\textbf{Answer:} We are pleased to learn from the meta-review ``\emph{Also, there has been some discussion about whether this paper fits topic-wise to PVLDB, which was ultimately answered affirmatively.}''

%We believe our work is relevant to the scope of VLDB due to the following reasons.

The well-known Kolmogorov-Smirnov (KS) test~\cite{klotz1967asymptotic} has been widely used in many studies closely related to VLDB. For example, Kifer~\textit{et~al.}~\cite{kifer2004detecting} apply the KS test to detect distribution drifts in data streams. Zheng~\textit{et~al.}~\cite{zheng2018order} apply the KS test to evaluate the performance of their proposed simulation framework of ridesharing order.
Agrawal~\textit{et~al.}~\cite{10.1145/1007568.1007632} propose a data encryption algorithm for database systems, and apply the KS test to verify the quality of the encrypted data. Zhao~\textit{et~al.}~\cite{10.1145/3183713.3183739} propose a sampling algorithm to speed up table join and apply the KS test to verify whether their  framework can generate samples from desired distributions.
Lee~\textit{et~al.}~\cite{lee2002learning} propose to conduct the KS test between a set of legitimate queries and a set of new coming queries to detect intrusion attacks to database systems. Buoncristiano~\textit{et~al.}~\cite{10.1145/2814710.2814714} propose an iterative algorithm to explore very large databases by using the KS test. With the surge in the applications of the KS test, there is
a great need for tools that help users analyze and understand the decisions of the KS test. Our work provides valuable contributions to this direction.

The major algorithmic contribution in this paper is on designing scalable data structures and algorithms that can search for the most comprehensible explanations efficiently, without conducting many KS tests.  Thus, it is a data processing and analysis task instead of just exploiting statistical properties.

To address the concern on the data set size, we conduct experiments on large synthetic datasets. In Section~\ref{subsec:exp_scale},
we interpret failed KS tests with test set sizes ranging from $10^4$ to $10^5$. Figure~\ref{fig:k_efficiency}b shows that our method is at least 10 times faster than the most efficient baseline method.


\subsection*{Comments by Reviewer \#3 (R3)}



\textbf{R3-Q1:} \textit{``(W1) The relationship to counterfactual interpretation is not completely transparent and convincing''}

\smallskip\noindent\textbf{Answer:} 
The concept of counterfactual explanations on failed KS tests is proposed following the principled idea of counterfactual explanation~\cite{moraffah2020causal}.
Please refer to our answer to question R1-Q6 for a more detailed discussion about causality discovery and counterfactual explanations.



\medskip

\textbf{R3-Q2:} \textit{``(W2) A convincing motivating example is missing''}

\smallskip\noindent\textbf{Answer:} A concrete motivating example using real data about COVID-19 is added to Section~\ref{sec:intro}.

\medskip
\textbf{R3-Q3:} \textit{``(W3) Experimental evaluation is not thoroughly convincing''}

\smallskip\noindent\textbf{Answer:} 
We conduct more extensive experiments in Section~\ref{sec:exp} to comprehensively compare MOCHE with six baseline methods. Among the 6 baseline methods, three are newly added to this revision.


We test all methods on 7 real world datasets of different application domains, such as COVID-19 cases, AWS CPU usages, and travel time. For each dataset except for the COVID-19 cases, we conduct KS tests with a variety of test set sizes, ranging from 100 to 200, 300, 1,000, 1,500, and 2,000.  We also construct large synthetic datasets to comprehensively evaluate the efficiency and scalability of our method.

We comprehensively evaluate the performance of all methods in four metrics, which are the size of explanations, the contrastivity of explanations, the effectiveness of explanations, and efficiency.
The experimental results show that our method MOCHE clearly outperforms all baseline methods in all experiments.
Even though some baseline methods have comparable contrastivity as our method (Section~\ref{sec:exp_effective}), as shown in Figure~\ref{fig:concise_sr_ais}, those methods tend to find a substantially larger subsets of the test set as explanations, which are not informative~\cite{grace, moraffah2020causal}.


\medskip
\textbf{R3-Q4:} \textit{``(W4) Presentation shall be improved by providing some more examples''}

\smallskip\noindent\textbf{Answer:} 
We add multiple new examples in our paper to better illustrate our motivation, problem formulation, and the proposed techniques. 
We add a concrete motivating example in Section~\ref{sec:intro}. 
We illustrate the difference between counterfactual explanations with different lexicographical orders 
and preference lists
in Example~\ref{ex:lexicographic_order}.  
%\todel{In the next paragraph following Example~\ref{ex:lexicographic_order}, we use a concrete example to explain choices of preference list.}
We add three running examples, Examples~\ref{ex:bounds}, ~\ref{ex:binary_search}, and~\ref{ex:interpretation_construction}, to clearly demonstrate the essential notations of our algorithm.

\medskip
\textbf{R3-Q5:} \textit{``(D1) While the idea of finding a minimal subset of data to be removed from the test set, taking into consideration some user-defined order, is clear, the relation to counterfactual explanations seems somewhat far-fetched to me. The point is that counterfactual explanations are based on causal relationships (as far as I understand), which I cannot see here. If some data points are removed from the test set to pass the KS test, this does not mean that the causes of abnormal behavior have been eliminated. This says only that those elements have been eliminated. For me the proposed solution would also be convincing without stressing the relationship to counterfactuals and just finding minimal subsets considering some preference order.
''}

\smallskip\noindent\textbf{Answer:} Please refer to our answer to the first question (R3-Q1).


\medskip
\textbf{R3-Q6:} \textit{``(D2) The experimental evaluation is not totally convincing and leaves some open issues. First, there are several experiments where the proposed MONCHI algorithm is not or only slightly better (in terms of quality) than some competitors, e.g., GRC in Fig. 2, GRD in Fig. 3, and GRC in Fig. 6. Second, only the runtime experiments use different lengths of the test sets. I think that it would also be interesting to use different test set sizes for the qualitative experiments.
''}

\smallskip\noindent\textbf{Answer:} 
%Please refer to our answer to the third question (R3-Q3).
Following this suggestion, we comprehensively evaluate the performance of all methods in four metrics, which are the size of explanations, the contrastivity of explanations, the effectiveness of explanations, and efficiency.
%As shown in Figures~\ref{fig:concise_sr_ais},~\ref{fig:ks_statistic} and \ref{fig:k_efficiency}, and Table~\ref{tbl:reverse_factor}, 
The experimental results show that our method MOCHE clearly outperforms all baseline methods in all experiments.
Even though some baseline methods have comparable contrastivity as our method (Section~\ref{sec:exp_effective}), as shown in Figure~\ref{fig:concise_sr_ais}, those methods tend to find a substantially larger subsets of the test set as explanations, which are not informative~\cite{grace, moraffah2020causal}.


\medskip
\textbf{R3-Q7:} \textit{``(D3) While the paper is generally very well written and nicely formalized, the technical parts are a bit dry and might be difficult to follow for some readers. I very much appreciate example 1 and 2 to illustrate some basic concepts, and strongly suggest to introduce more examples and if possible illustrations in the technical part of the paper (Sec. 4 and 5). While technically sound, a running example might significantly improve the readability. 
''}

\smallskip\noindent\textbf{Answer:} %Please refer to our answer to the fourth question (R3-Q4).
We add three running examples, Examples~\ref{ex:bounds}, ~\ref{ex:binary_search}, and~\ref{ex:interpretation_construction}, to clearly demonstrate the essential notations of our algorithm.

\medskip
\textbf{R3-Q8:} \textit{``(D4) Similarly to point D3, it would be helpful if high-level intuitive descriptions of the theorems could be provided.
''}

\smallskip\noindent\textbf{Answer:} 
The high-level intuitive descriptions of Theorems~\ref{theorem:l_u_bound_fast_check},~\ref{theorem:necessary_condition}, and~\ref{theorem:correctness_algorithm_interpretation_superset_check} are added to the paragraphs right before each theorem.


\medskip
\textbf{R3-Q9:} \textit{``(D5) The last paragraph in Sec. 3.3 briefly explains different preference orders. It would be nice to elaborate a bit more on this, showing perhaps some more concrete examples of preference orders. It might also be considered to move this discussion together with concrete examples to the introduction as a motivation for the work.
''}

\smallskip\noindent\textbf{Answer:} 
In this revision, we change the motivation example to one using COVID-19 real data.  Example~\ref{ex:lexicographic_order} illustrates two possible preference lists and compares the corresponding explanations.

